Pre-Trained Language Models for Interactive Decision-Making

Language model (LM) pre-training is useful in many language processing tasks. But can pre-trained LMs be further leveraged for more general machine learning problems? We propose an approach for using LMs to scaffold learning and generalization in general sequential decision-making problems. In this approach, goals and observations are represented as a sequence of embeddings, and a policy network initialized with a pre-trained LM predicts the next action. We demonstrate that this framework enables effective combinatorial generalization across different environments and supervisory modalities. We begin by assuming access to a set of expert demonstrations, and show that initializing policies with LMs and fine-tuning them via behavior cloning improves task completion rates by 43.6% in the VirtualHome environment. Next, we integrate an active data gathering procedure in which agents iteratively interact with the environment, relabel past "failed" experiences with new goals, and update their policies in a self-supervised loop. Active data gathering further improves combinatorial generalization, outperforming the best baseline by 25.1%. Finally, we explain these results by investigating three possible factors underlying the effectiveness of the LM-based policy. We find that sequential input representations (vs. fixed-dimensional feature vectors) and LM-based weight initialization are both important for generalization. Surprisingly, however, the format of the policy inputs encoding (e.g. as a natural language string vs. an arbitrary sequential encoding) has little influence. Together, these results suggest that language modeling induces representations that are useful for modeling not just language, but also goals and plans; these representations can aid learning and generalization even outside of language processing.

==> fig/13analysis.tex <==
\begin{figure*}[t]
\centering
\hfill
\begin{minipage}{0.44\textwidth}
    \centering
    \small
      \centering
      \addtolength{\tabcolsep}{-3.5pt}
      \scalebox{0.8}{
      \begin{tabular}{lcccccccc}
    \toprule
    \bf Methods & \multicolumn{6}{c}{\bf Number of Demos} \\
    % \cline{2-7}
    \cmidrule(lr){2-7}
    & \bf 100 & \bf 500 & \bf 1K & \bf 5K & \bf 10K & \bf 20K \\
    
    \midrule
    
    \bf \modelname-Text (Ours) & \bf 8.8 & \bf 22.2 & 26.8 & 46.0  & \bf 58.2  & 58.2 \\
    % \bf \modelname-Index (Ours) & 6.4   & 18.0  & 18.8  & 32.8  & 52.2 & 57.8 \\
    \bf \modelname-Index (Ours) & 6.4   & 18.0  & 18.8  & 45.5  & 54.6 & 57.8 \\
    \bf \modelname-Unnatural (Ours) &  6.8 & 18.6 & \bf 27.0 & \bf 47.2 & 55.8 & \bf 58.8 \\
    \bottomrule
  \end{tabular}
    }
    \vspace{-5pt}
    \captionof{table}{\small{\textbf{Success rates of policies trained with different input encodings in the \emph{Novel Tasks} setting on VirtualHome.} The text encoding is most sample-efficient, but all models converge to similar performance given sufficient training data.}}
    \label{exp:learnedemb}
\end{minipage}
\hfill \hfill
\begin{minipage}{0.54\textwidth}
    \centering
    \small
      \centering
      \addtolength{\tabcolsep}{-3.5pt}
      \scalebox{0.8}{
    \begin{tabular}{llcccccc}
    \toprule
    \bf Tasks & \bf Methods & \multicolumn{5}{c}{\bf Number of Demos} \\
     \cmidrule(lr){3-7}
    & &  \bf 100 & \bf 500 & \bf 1K & \bf 5K & \bf 10K \\
    
    \midrule
    
    \multirow{2}{*}{\bf GoToRedBall} 
    & \bf \modelname-Text (Ours) & \bf 93.9 & \bf 99.4 & 99.7 & \bf 100.0 & \bf 100.0 \\
    & \bf \modelname-Conv (Ours) & 92.5 & 98.8 & \bf 100.0 & \bf 100.0 & \bf 100.0 \\ % old
    % & \bf \modelname-Grid (Ours) & 89.6 & 98.9 & 99.6 & 100.0 & 100.0 \\ % new
    % & \bf \modelname-Grid (Ours) & 91.8 & \bf 99.4 & \bf 100.0 & 99.8 & 99.8 \\ % new best
    
    
    \midrule
    
    \multirow{2}{*}{\bf GoToLocal} 
    & \bf \modelname-Text (Ours) &  64.6 & \bf 97.9 & \bf 99.0 & 99.5 & 99.5 \\
    & \bf \modelname-Conv (Ours) & \bf 69.5 & 86.0 & 98.2 & \bf 99.9 & \bf 99.9 \\ % old
    % & \bf \modelname-Grid (Ours) &  43.2 & 81.1 & 96.1 & \bf 99.9 & \bf 99.8 \\ % new
    % & \bf \modelname-Grid (Ours) & 45.6 & 78.4 & 80.8 & 100.0 & 99.8 \\ % new best
    
    
    \midrule
    
    \multirow{2}{*}{\bf PickupLoc} 
    & \bf \modelname-Text (Ours) & \bf 28.7 & \bf 73.4 & \bf 99.0 & \bf 99.6 & 99.8 \\
    & \bf \modelname-Conv (Ours) & 25.0 & 58.8 & 95.1 & \bf 99.6 & \bf 100.0 \\ % old
    % & \bf \modelname-Grid (Ours) & 29.3 & 62.5 & 97.4 & 99.2 & 99.2 \\ % new
    % & \bf \modelname-Grid (Ours) & 27.2 & 64.6 & 94.7 & 99.2 & 99.3\\ % new best
    
    
    \midrule
    
    \multirow{2}{*}{\bf PutNextLocal} 
    & \bf \modelname-Text (Ours) & 11.1 & \bf 93.0 & \bf 93.2 & \bf 98.9 & \bf 99.9 \\
    & \bf \modelname-Conv (Ours) & \bf 17.9 & 53.6 & 91.3 & 97.7 & 99.5 \\ % old
    % & \bf \modelname-Grid (Ours) & 16.6 & 46.9 & 95.5 & 99.8 & 86.9 \\ % new
    % & \bf \modelname-Grid (Ours) & \bf 15.0 & 46.9 & 76.3 & 99.8 & 86.9 \\ % new best
    
    
    \bottomrule
  \end{tabular}
    }
    \vspace{-5pt}
    \captionof{table}{\small \textbf{Success rate of policies trained with \emph{text encoding} vs. \emph{convolutional encoding} on BabyAI.} The text encoding is more sample-efficient, but both models converge to near perfect performance given sufficient training data.}
  \label{tbl:babyai_encodings}
\end{minipage}

\vspace{-10pt}
\end{figure*}





==> fig/1baselines.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.6\textwidth]{fig/files/1baselines.pdf}
\end{center}
\vspace{-10pt}
\caption{\small{\textbf{Comparisons of the proposed method and baselines on VirtualHome.}
All the methods are trained on expert data using imitation learning.
% Results on three testing settings are reported.
\emph{MLP-1}, \emph{MLP}, and \emph{LSTM} are baselines without using the pre-trained LM. The proposed method, \emph{\modelname-Text (Ours)}, outperforms all baselines.}}
\label{exp:result_baselines}
\vspace{-10pt}
\end{figure}

% comparison of the propose method on the default setting and other ablation settings.
% in distribution, flatter and flatter






==> fig/2active_data_provider.tex <==
\begin{table*}[t]
\small
  \caption{\small \modelname-ADG can be used as an policy initializer for online RL or a data provider for offline RL.}
  \vspace{-5pt}
  \label{exp:provider}
  \centering
  \setlength{\tabcolsep}{0.5em}
  \scalebox{0.9}{
  \begin{tabular}{lccccc}
    \toprule
    & \bf {In-Distribution} & \bf {Novel Scenes} & \bf \shortstack{Novel Tasks} \\
    \midrule
    
    \bf \modelname-ADG (Ours) & 46.70 $\pm$ 2.73 & \bf 32.16 $\pm$ 3.32 & 25.49 $\pm$ 4.07  \\
    \bf PPO (Init from \modelname-ADG) & \bf 53.73 $\pm$ 3.54 & 30.20 $\pm$ 3.43 & \bf 27.84 $\pm$ 2.66 \\
    \bf DT~\citep{chen2021decision} (\modelname-ADG Data) & 42.40 $\pm$ 1.47 & 21.60 $\pm$ 2.48 & 16.80 $\pm$ 1.02 \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-5pt}
\end{table*}






% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.6\textwidth]{fig/files/1provider.pdf}
% \end{center}
% \vspace{-10pt}
% \caption{\small \modelname-ADG can be used as an initializer for online RL, or a data provider for offline RL.}
% \label{exp:provider}
% \vspace{-5pt}
% \end{figure}


==> fig/ablation_results.tex <==

\begin{figure}[t]
\begin{center}
\includegraphics[width=1\textwidth]{fig/files/2ablation.pdf}
\end{center}
\vspace{-10pt}
\caption{\small{ablation.}}
\label{fig:result}
\end{figure}


==> fig/environment.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=1\textwidth]{fig/files/environment.pdf}
\end{center}
\vspace{-13pt}
\caption{\small VirtualHome is a 3D interactive environment simulating household activities. It provides a symbolic graph representation of the partial observation. The action space changes over time based on the observation.}
\vspace{-17pt}
\label{fig:environment}
\end{figure*}


==> fig/random_result.tex <==

\begin{figure}[t]
\begin{center}
\includegraphics[width=1\textwidth]{fig/files/1random.pdf}
\end{center}
\vspace{-10pt}
\caption{\small{random.}}
\label{fig:result}
\end{figure}



==> fig/teaser.tex <==
% \begin{figure*}
% \begin{center}
% \includegraphics[width=1\linewidth]{fig/files/teaser2.pdf}
% \end{center}
% \vspace{-10pt}
% \caption{\textbf{(a) Overview of the proposed method.} We encode the inputs to the policy --- including observations, goals, and action histories --- as templated English phrases. The phrases are sent to an embedding layer and a pre-trained language model to predict the subsequent action. The embedding layer $f_{\phi}$ can either be a embedding layer of a pre-trained language model (Experiment 1) or be a learned embedding layer (Experiment 2).
% \textbf{(b) Results.} We summarize the main results of Experiment 1 (``Transformer from scratch'' and ``Pretrained transformer (natural encoding)''), Experiment 2A (``Pretrained transformer (random encoding)'') and Experiment 2B (``Pretrained transformer (learned encoding)'').
% % \jda{we should try to squeeze in a bar chart summarizing the main results: on the hardest OOD split, one bar each for transformer-scratch, transformer-pretrained, trainsformer-scrambled-vocab, transformer-learned-adapter} \jda{The ``parital observation'' box makes this look like it's just a bag of words encoding. We're doing something more structured, right? Can we make this clearer?} \jda{since this is the teaser and experiment 2 is about other encoding schemes, can we add a detail to one of the ``serialize'' boxes that shows the other two encodings?}
% }
% \label{fig:teaser}
% \vspace{-15pt}
% \end{figure*}


==> table/2active_data_baselines.tex <==
\begin{table*}[t]
\small
  \caption{\small{\textbf{Comparisons of methods without using expert data.} Results on three VirtualHome testing settings are reported. The proposed method with active data gathering, \emph{\modelname-ADG (Ours)}, outperforms all baselines.}}
  \vspace{-5pt}
  \label{exp:baselines}
  \centering
  \setlength{\tabcolsep}{0.5em}
  \scalebox{0.9}{
  \begin{tabular}{lccccc}
    \toprule
    & \bf {In-Distribution} & \bf {Novel Scenes} & \bf \shortstack{Novel Tasks} \\
    \midrule
    
    \bf Random  & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00  \\
    \bf Goal-Object & 0.78 $\pm$ 0.48 & 0.00 $\pm$ 0.00 & 0.39 $\pm$ 0.39 \\
    \bf PPO~\citep{schulman2017proximal} & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 \\
    \bf DQN+HER~\citep{andrychowicz2017hindsight}  & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 \\
    \bf \modelname-ADG (Ours) & \bf 46.70 $\pm$ 2.73 & \bf 32.16 $\pm$ 3.32 & \bf  25.49 $\pm$ 4.07  \\
    
    \bottomrule
  \end{tabular}
  }
  \vspace{-5pt}
\end{table*}



==> table/2active_data_human.tex <==
% \begin{table}[t]
% \small
%   \caption{\small 
%          \hl{\textbf{Comparisons of the proposed method and baselines on real human language tasks.} 
%          \modelname-ADG (Ours) can generalize to novel language goals written by humans in the \emph{Real-Human-Goal} setting.}
%          }
%         \label{exp:human}
%   \centering
%   \setlength{\tabcolsep}{0.5em}
%   \scalebox{0.9}{
%   \begin{tabular}{lccccc}
%     \toprule
%     & \bf {In-Distribution} & \bf {Real-Human-Goal}  \\
%     \midrule
    
%     \bf \modelname-ADG (Ours) & \bf 46.70 $\pm$ 2.73 & \bf 41.17 $\pm$ 1.04 \\
%     \bf \modelname-ADG (No-Pretrain) & 43.13 $\pm$ 3.82 & 30.50 $\pm$ 1.07 \\
%     \bf \modelname-ADG (No-FT) & 28.23 $\pm$ 3.90 & 22.85 $\pm$ 0.91 \\
%     \bf \modelname-ADG (No-Seq) & 24.31 $\pm$ 1.33 & 23.09 $\pm$ 0.18 \\
    
%     \bottomrule
%   \end{tabular}
%   }
% \vspace{-5pt}
% \end{table}



\begin{table}[h]
\small
  \caption{\small 
         \textbf{Results of the proposed method on different test settings.} 
         \modelname-ADG (Ours) can generalize to novel language goals written by humans in the \emph{Real-Human-Goal} setting.
         }
        \label{exp:human}
  \centering
%   \setlength{\tabcolsep}{0.5em}
  \scalebox{0.9}{
  \begin{tabular}{lccccccc}
    \toprule
    & \bf {In-Distribution} & \bf {Novel Scenes} & \bf \shortstack{Novel Tasks} & \bf {Real-Human-Goal}  \\
    \midrule
    \bf \modelname-ADG (Ours) & \bf 46.7 $\pm$ 2.7 & \bf 32.2 $\pm$ 3.3 & \bf  25.5 $\pm$ 4.1 & \bf 41.2 $\pm$ 1.04 \\
    \bottomrule
  \end{tabular}
  }
% \vspace{-5pt}
\end{table}















==> table/3seq_input.tex <==

% \begin{table}[t]
% \small
% \vspace{-5pt}
%   \caption{\small 
%          \textbf{Results of removing the sequential inputs and removing pre-trained weights on novel tasks.} ``No-Seq'' is the pre-trained language model using non-sequential inputs. ``No-Pretrain'' has the same Transformer architecture with the proposed method, ``ML (Ours)'', but without using the pre-trained weights.
%          }
%         \label{exp:noseq}
%   \centering
%   \scalebox{0.9}{
%   \begin{tabular}{lccc}
%     \toprule
%     % & \bf \shortstack{Novel Goal \\ Combinations} & \bf \bf \shortstack{Novel Scene \\ Combinations} & \bf Normal \\
%     & \bf No-Seq & \bf No-Pretrain & \bf ML (Ours) \\
%     \midrule
%     1K Training Data & 1.60 $\pm$ 1.02 & 20.20 $\pm$ 3.86 & 26.80 $\pm$ 1.93 \\
%     10K Training Data & 2.00 $\pm$ 0.63 & 47.00 $\pm$ 2.83 & 58.20 $\pm$ 2.32\\
%     \bottomrule
%   \end{tabular}
%   }
% \end{table}





% \begin{table}[t]
% \small
% \vspace{-5pt}
%   \caption{\small 
%          \textbf{Results of removing the sequential inputs and removing pre-trained weights on novel tasks.} ``No-Seq'' is the pre-trained language model using non-sequential inputs. ``No-Pretrain'' has the same Transformer architecture with the proposed method, ``ML (Ours)'', but without using the pre-trained weights.
%          }
%         \label{exp:noseq}
%   \centering
%   \scalebox{0.9}{
%   \begin{tabular}{llll}
%     \toprule
%     & \bf 1K Training Demos & \bf 10K Training Demos \\
%     \midrule
    
%     \bf No-Seq  & 1.60 $\pm$ 1.02 & 2.00 $\pm$ 0.63 \\
%     \bf No-Pretrain & 20.20 $\pm$ 3.86 & 47.00 $\pm$ 2.83 \\
%     \bf No-FineTune & 6.00 $\pm$ 1.78 & 17.0 $\pm$ 2.89 \\
%     \bf ML (Ours) & 26.80 $\pm$ 1.93 & 58.20 $\pm$ 2.32 \\
%     \bottomrule
%   \end{tabular}
%   }
% \vspace{-10pt}
% \end{table}






% \begin{table}[t]
% \small
% \vspace{-5pt}
%   \caption{\small 
%          \textbf{Results of removing the sequential inputs and removing pre-trained weights on novel tasks.} ``No-Seq'' is the pre-trained language model using non-sequential inputs. ``No-Pretrain'' has the same Transformer architecture with the proposed method, ``ML (Ours)'', but without using the pre-trained weights.
%          }
%         \label{exp:noseq}
%   \centering
%   \scalebox{0.9}{
%   \begin{tabular}{llll}
%     \toprule
%     & \bf In-Distribution & \bf Novel Scenes & \bf Novel Tasks \\
%     \midrule
    
    
%     \bf No-Seq  & 74.00 $\pm$ 2.28 & 28.80 $\pm$ 2.13 & 2.00 $\pm$ 0.63 \\
%     \bf No-Pretrain & \textbf{87.80 $\pm$ 2.03} & \textbf{42.80 $\pm$ 3.91} & 47.00 $\pm$ 2.83 \\
%     \bf No-FineTune & 51.20 $\pm$ 4.53 & 10.40 $\pm$ 3.61 & 17.0 $\pm$ 2.89 \\
%     \bf ML (Ours) & 87.60 $\pm$ 1.85 & 39.00 $\pm$ 1.78 & \textbf{58.20 $\pm$ 2.32} \\
%     \bottomrule
%   \end{tabular}
%   }
% \vspace{-10pt}
% \end{table}



\begin{table}[t]
\small
\vspace{-5pt}
  \caption{\small 
         \textbf{Results of removing the sequential inputs and removing pre-trained weights on novel tasks.} ``No-Seq'' is the pre-trained language model using non-sequential inputs. ``No-Pretrain'' has the same Transformer architecture with the proposed method, ``ML (Ours)'', but without using the pre-trained weights.
         }
        \label{exp:noseq}
  \centering
  \scalebox{0.9}{
  \begin{tabular}{llll}
    \toprule
    & \bf In-Distribution & \bf Novel Tasks \\
    \midrule
    
    \bf ML (Ours) & 87.60 $\pm$ 1.85 & \textbf{58.20 $\pm$ 2.32} \\
    \bf No-Pretrain & \textbf{87.80 $\pm$ 2.03} &  47.00 $\pm$ 2.83 \\
    \bf No-FineTune & 51.20 $\pm$ 4.53 & 17.0 $\pm$ 2.89 \\
    \bf No-Seq  & 74.00 $\pm$ 2.28 & 2.00 $\pm$ 0.63 \\
    \bottomrule
  \end{tabular}
  }
\vspace{-10pt}
\end{table}


==> table/4templates.tex <==

\begin{table}[t]
\small
  \caption{\small 
         \textbf{Results of using different templates.}
         }
        \label{exp:templates}
  \centering
  \scalebox{0.9}{
  \begin{tabular}{lccc}
    \toprule
    % & \bf \shortstack{Novel Goal \\ Combinations} & \bf \bf \shortstack{Novel Scene \\ Combinations} & \bf Normal \\
    & \bf T1 & \bf T2 & \bf T3 (Ours) \\
    \midrule
    1K Training Data & 30.40 $\pm$ 2.57 & 31.60 $\pm$ 3.00 & 28.80 $\pm$ 1.95 \\
    10K Training Data & 42.40 $\pm$ 2.87 & 37.20 $\pm$ 1.26 & 58.20 $\pm$ 2.32\\
    10K Training Data & - & - & 58.20 $\pm$ 2.32\\
    \bottomrule
  \end{tabular}
  }
\end{table}


==> table/5babiai.tex <==
% % \begin{table}[t]
% % \small
% % \vspace{-5pt}
% %   \caption{\small 
% %          \textbf{babyai}
% %          }
% %         \label{exp:noseq}
% %   \centering
% %   \scalebox{0.9}{
% %   \setlength{\tabcolsep}{0.3em}
% %   \begin{tabular}{lcccc}
% %     \toprule
% %     \bf Levels & \bf $\#$Demos 
% %     & \multicolumn{3}{c}{\bf Success Rate} \\
% %     \cline{3-5}
% %     & & \bf BabyAI & \bf \modelname-Grid & \bf \modelname-Text (Ours) \\
    
% %     \midrule
    
% %     \multirow{4}{*}{\bf GoToRedBall} 
% %     &1K \\
% %     &5K & 99.3 \\
% %     &10K & 99.8  \\
% %     &50K & 100  \\
% %     &100K & 100  \\
    
% %     \midrule
    
% %     \multirow{4}{*}{\bf GoToLocal} 
% %     &1K \\
% %     &5K & 84.2 \\
% %     &10K & 94.2  \\
% %     &50K & 99.8  \\
% %     &100K & 99.9 \\
    
% %     \midrule
    
% %     \multirow{4}{*}{\bf PutNextLocal} 
% %     &1K \\
% %     &5K & 12.5  \\
% %     &10K & 24.9  \\
% %     &50K & 88.6 \\
% %     &100K & 99.5  \\
    
% %     \midrule
    
% %     \multirow{4}{*}{\bf PickupLoc} 
% %     &1K \\
% %     &5K & 60.3  \\
% %     &10K & 74.9 \\
% %     &50K & 97.0 \\
% %     &100K & 98.6 \\
    
% %     \bottomrule
% %   \end{tabular}
% %   }
% % \end{table}


% \begin{table}[t]
% \small
% \vspace{-5pt}
%   \caption{\small 
%          \textbf{babyai}
%          }
%         \label{exp:noseq}
%   \centering
%   \scalebox{0.9}{
%   \setlength{\tabcolsep}{0.5em}
%   \begin{tabular}{llcccccc}
%     \toprule
%     \bf Levels & \multicolumn{6}{c}{\bf Number of Demos} \\
%     \cline{2-8}
%     & & 500 & 1K & 5K & 10K & 50K & 100K \\
    
%     \midrule
    
%     \multirow{3}{*}{\bf GoToRedBall} 
%     & \bf BabyAI & 96.0 & 99.0 & 99.3 & 99.8 & 100.0 & 100.0 \\
%     & \bf \modelname-Grid & & & \\
%     & \bf \modelname-Text (Ours) & & & \\
    
%     \midrule
    
%     \multirow{3}{*}{\bf GoToLocal} 
%     & \bf BabyAI & 82.4 & 98.6 & 84.2 & 94.2 & 99.8 & 99.9 \\
%     & \bf \modelname-Grid & & & \\
%     & \bf \modelname-Text (Ours) & & & \\
    
%     \midrule
    
%     \multirow{3}{*}{\bf PutNextLocal} 
%     & \bf BabyAI & 16.8 & 43.4 & 12.5 & 24.9 & 88.6 & 99.5 \\
%     & \bf \modelname-Grid & & & \\
%     & \bf \modelname-Text (Ours) & & & \\
    
%     \midrule
    
%     \multirow{3}{*}{\bf PickupLoc} 
%     & \bf BabyAI & 58.0 & 93.3 & 60.3 & 74.9 & 97.0 & 98.6 \\
%     & \bf \modelname-Grid & & & \\
%     & \bf \modelname-Text (Ours) & & & \\
    
%     \bottomrule
%   \end{tabular}
%   }
% \end{table}




% \begin{table}[t]
% \small
% \vspace{-5pt}
%   \caption{\small 
%          \textbf{babyai}
%          }
%         \label{tbl:babyai}
%   \centering
%   \scalebox{0.9}{
%   \setlength{\tabcolsep}{0.3em}
%   \begin{tabular}{lcccc}
%     \toprule
%     \bf Levels & \bf $\#$Demos 
%     & \multicolumn{3}{c}{\bf Success Rate} \\
%     \cline{3-5}
%     & & \bf BabyAI & \bf \modelname-Grid & \bf \modelname-Text (Ours) \\
    
%     \midrule
    
%     \multirow{4}{*}{\bf GoToRedBall} 
%     &1K \\
%     &5K & 99.3 \\
%     &10K & 99.8  \\
%     &50K & 100  \\
%     &100K & 100  \\
    
%     \midrule
    
%     \multirow{4}{*}{\bf GoToLocal} 
%     &1K \\
%     &5K & 84.2 \\
%     &10K & 94.2  \\
%     &50K & 99.8  \\
%     &100K & 99.9 \\
    
%     \midrule
    
%     \multirow{4}{*}{\bf PutNextLocal} 
%     &1K \\
%     &5K & 12.5  \\
%     &10K & 24.9  \\
%     &50K & 88.6 \\
%     &100K & 99.5  \\
    
%     \midrule
    
%     \multirow{4}{*}{\bf PickupLoc} 
%     &1K \\
%     &5K & 60.3  \\
%     &10K & 74.9 \\
%     &50K & 97.0 \\
%     &100K & 98.6 \\
    
%     \bottomrule
%   \end{tabular}
%   }
% \end{table}




\begin{table}[t]
\caption{\small 
         \textbf{Success rates of the proposed method vs. baseline on four BabyAI tasks.}
         All the methods are trained on offline expert data using imitation learning.
        \emph{\modelname-Text (Ours)} outperforms \citep{hui2020babyai}, the method used in the original paper. 
        %  This difference is more pronounced when fewer training datapoints are provided.
         }
\label{exp_tbl:babyai_baselines}
\small
  \centering
  \scalebox{0.9}{
%   \setlength{\tabcolsep}{0.4em}
  \begin{tabular}{llcccccc}
    \toprule
    \bf Tasks & \bf Methods & \multicolumn{5}{c}{\bf Number of Demos} \\
     \cmidrule(lr){3-7}
    & &  \bf 100 & \bf 500 & \bf 1K & \bf 5K & \bf 10K \\
    
    \midrule
    
    \multirow{2}{*}{\bf GoToRedBall} 
    & \bf \citep{hui2020babyai} & 81.0 & 96.0 & 99.0 & 99.5 & 99.9 \\
    % & \bf \modelname-Grid & 92.5 & 98.8 & \bf 100.0 & \bf 100.0 & \bf 100.0 \\ % old
    & \bf \modelname-Text (Ours) & \bf 93.9 & \bf 99.4 & \bf 99.7 & \bf 100.0 & \bf 100.0 \\
    
    \midrule
    
    \multirow{2}{*}{\bf GoToLocal} 
    & \bf \citep{hui2020babyai} & 55.9 & 84.3 & 98.6 & \bf 99.9 & 99.8 \\
    % & \bf \modelname-Grid & \bf 69.5 & 86.0 & 98.2 & \bf 99.9 & \bf 99.9 \\
    & \bf \modelname-Text (Ours) & \bf 64.6 & \bf 97.9 & \bf 99.0 & 99.5 & 99.5 \\
    
    \midrule
    
    \multirow{2}{*}{\bf PickupLoc} 
    & \bf \citep{hui2020babyai} & 28.0 & 58.0 & 93.3 & 97.9 & \bf 99.8 \\
    % & \bf \modelname-Grid & 25.0 & 58.8 & 95.1 & \bf 99.6 & \bf 100.0 \\
    & \bf \modelname-Text (Ours) & \bf 28.7 & \bf 73.4 & \bf 99.0 & \bf 99.6 & \bf 99.8 \\
    
    \midrule
    
    \multirow{2}{*}{\bf PutNextLocal} 
    & \bf \citep{hui2020babyai} & \bf 14.3 & 16.8 & 43.4 & 81.2 & 97.7 \\
    % & \bf \modelname-Grid & \bf 17.9 & 53.6 & 91.3 & 97.7 & 99.5 \\
    & \bf \modelname-Text (Ours) & 11.1 & \bf 93.0 & \bf 93.2 & \bf 98.9 & \bf 99.9 \\
    
    \bottomrule
  \end{tabular}
  }
\end{table}




% \begin{table}[t]
% \small
%   \caption{\small 
%          \textbf{Comparisons of the proposed method and baselines on different testing subsets on BabyAI.}
%          }
%   \vspace{-5pt}
%   \label{tbl:babyai}
%   \centering
%   \scalebox{0.9}{
%   \setlength{\tabcolsep}{0.4em}
%   \begin{tabular}{llcccccc}
%     \toprule
%     \bf Tasks & \bf Methods & \multicolumn{5}{c}{\bf Number of Demos} \\
%      \cmidrule(lr){3-7}
%     & &  \bf 100 & \bf 500 & \bf 1K & \bf 5K & \bf 10K \\
    
%     \midrule
    
%     \multirow{3}{*}{\bf GoToRedBall} 
%     & \bf \citep{hui2020babyai} & 81.0 & 96.0 & 99.0 & 99.5 & 99.9 \\
%     & \bf \modelname-Grid & 92.5 & 98.8 & \bf 100.0 & \bf 100.0 & \bf 100.0 \\ % old
%     & \bf \modelname-Grid (Ours) & 91.8 & \bf 99.4 & \bf 100.0 & \bf 100.0 & \bf 100.0 \\ % (best)
%     % & \bf \modelname-Grid (Ours) & 89.6 & 98.9 & 99.6 & \bf 100.0 & \bf 100.0 \\
%     & \bf \modelname-Text (Ours) & \bf 93.9 & \bf 99.4 & 99.7 & \bf 100.0 & \bf 100.0 \\
    
%     \midrule
    
%     \multirow{3}{*}{\bf GoToLocal} 
%     & \bf \citep{hui2020babyai} & 55.9 & 84.3 & 98.6 & \bf 99.9 & 99.8 \\
%     & \bf \modelname-Grid & \bf 69.5 & 86.0 & 98.2 & \bf 99.9 & \bf 99.9 \\
%     & \bf \modelname-Grid (Ours) & 45.6 & 78.4 & 80.8 & 99.8 & 98.2 \\
%     & 2 & 43.2 & 81.1 & 96.1 & 99.9 & 99.6 \\
%     & \bf \modelname-Text (Ours) & 64.6 & \bf 97.9 & \bf 99.0 & 99.5 & 99.5 \\
    
%     \midrule
    
%     \multirow{3}{*}{\bf PickupLoc} 
%     & \bf \citep{hui2020babyai} & 28.0 & 58.0 & 93.3 & 97.9 & 99.8 \\
%     & \bf \modelname-Grid & 25.0 & 58.8 & 95.1 & \bf 99.6 & \bf 100.0 \\
%     & \bf \modelname-Grid (Ours) & 27.2 & 64.6 & 94.7 & 98.3 & 99.2 \\
%     & 2 & 29.3 & 62.5 & 97.4 & 99.2 & 98.4 \\
%     & \bf \modelname-Text (Ours) & \bf 28.7 & \bf 73.4 & \bf 99.0 & \bf 99.6 & 99.8 \\
    
%     \midrule
    
%     \multirow{3}{*}{\bf PutNextLocal} 
%     & \bf \citep{hui2020babyai} & 14.3 & 16.8 & 43.4 & 81.2 & 97.7 \\
%     & \bf \modelname-Grid & \bf 17.9 & 53.6 & 91.3 & 97.7 & 99.5 \\
%     & \bf \modelname-Grid (Ours) & 15.0 & 15.7 & 76.3 & 99.5 & 19.7 \\
%     & 2 & 16.6 & 46.9 & 95.5 & 99.4 & 83.0 \\
%     & \bf \modelname-Text (Ours) & 11.1 & \bf 93.0 & \bf 93.2 & \bf 98.9 & \bf 99.9 \\
    
%     \bottomrule
%   \end{tabular}
%   }
% \vspace{-15pt}
% \end{table}




==> table/comparison_generalization.tex <==

% \begin{table*}[h]
% \caption{\small{Comparisons of the generalization ability of the proposed method and baselines on unseen test subsets. Single agent setting. 100 valid trajectories}}
% \vspace{-5pt}
% \label{tbl:baselines_generalization}
% \begin{center}
% \small
% \setlength{\tabcolsep}{3pt}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{l|ccc|ccc|ccc}
% \toprule
% & \multicolumn{3}{c}{\bf Normal } &  \multicolumn{3}{c}{\bf Less subgoals } & \multicolumn{3}{c}{\bf More subgoals } \\
% \midrule
% & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ \\
% \midrule
% MLP-1 + MLP  & 26.600 & 3.756 & 84.970	 & 62.000 & 1.240 & 52.760	 & 9.000 & 6.150 & 96.985  \\
% MLP-N + MLP  & 28.400 & 4.264 & 87.452	& 69.000 & 1.380 & 53.670	 & 7.000 & 6.440 & 98.490 \\
% MLP-N + LSTM  & 40.600 & 5.708 & 75.522	 & 61.000 & 1.220 & 48.340	 & 22.500 & 10.070 & 91.855 \\
% \midrule
% MLP-N + LLM  (scratch) & 49.200 & 6.232 & 74.156	& 93.000 & 1.860 & 24.200	& 19.500 & 11.010 & 94.510	\\
% \midrule
% MLP-N + LLM  & 60.400 & 6.272 & 61.902	 & 96.000 & 1.920 & 17.450	 & 34.500 & 10.670 & 85.100 \\
% \midrule
% MLP-N + LLM + Mes & 73.000 & 6.876 & 56.736	 & 96.000 & 1.920 & 16.030	 & 55.500 & 12.330 & 80.095 \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table*}






% \begin{table*}[h]
% \caption{\small{Comparisons of the generalization ability of the proposed method and baselines on unseen test subsets. Single agent setting. 100 valid trajectories}}
% \vspace{-5pt}
% \label{tbl:baselines_generalization}
% \begin{center}
% \small
% \setlength{\tabcolsep}{3pt}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{l|ccc|ccc|ccc}
% \toprule
% & \multicolumn{3}{c}{\bf Abnormal init } &  \multicolumn{3}{c}{\bf Unused final } & \multicolumn{3}{c}{\bf Abnormal init+Unused final } \\
% \midrule
% & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ \\
% \midrule
% MLP-1 + MLP  & 17.000 & 3.940 & 89.980	& 0.000 & 0.000 & 100.000	& 0.000  & 0.000 & 100.000 \\
% MLP-N + MLP  & 16.000 & 4.100 & 94.830	& 0.000 & 0.000 & 100.000	 & 0.000 & 0.000 & 100.000 \\
% MLP-N + LSTM  &  13.000 & 3.780 & 94.070	& 0.000 & 0.120 & 100.000	& 0.000 & 0.080 & 100.000 \\
% \midrule
% MLP-N + LLM  (scratch) & 36.000  & 5.900 & 82.340	 & 0.000 &  0.700 & 100.000	& 1.000 &  0.380 & 99.480 	\\
% \midrule
% MLP-N + LLM  & 45.000 & 6.280 & 80.790	& 6.000 & 1.280 & 97.540	& 1.000 & 0.520 & 99.350	\\
% \midrule
% MLP-N + LLM + Mes & 66.000 & 7.000 & 62.810	 & 12.000 & 3.140 & 94.590	 & 12.000 & 1.880 & 93.170 \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table*}












% \begin{table*}[t]
% \caption{\small{Comparisons of the generalization ability of the proposed method and baselines on unseen test subsets. Single agent setting. 100 valid trajectories}}
% \label{tbl:baselines_generalization}
% \begin{center}
% \small
% \setlength{\tabcolsep}{3pt}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}{l|c|c|c|c|c|c}
% \toprule
% Methods & & \bf MLP-1 + MLP & \bf MLP-N + MLP & \bf MLP-N + LSTM & \bf MLP-N + LLM  (scratch) & \bf MLP-N + LLM (ft) \\
% \midrule
% \multirow{3}{*}{\bf Normal}
%     & Success $\uparrow$ \\
%     & Reward  $\uparrow$ \\
%     & Steps $\downarrow$ \\
% \midrule
% \multirow{3}{*}{\bf Less subgoals}
%     & Success $\uparrow$ \\
%     & Reward  $\uparrow$ \\
%     & Steps $\downarrow$ \\
% \midrule
% \multirow{3}{*}{\bf More subgoals}
%     & Success $\uparrow$ \\
%     & Reward  $\uparrow$ \\
%     & Steps $\downarrow$ \\
% \midrule
% \multirow{3}{*}{\bf Zero-shot}
%     & Success $\uparrow$ \\
%     & Reward  $\uparrow$ \\
%     & Steps $\downarrow$ \\
% \midrule
% \multirow{3}{*}{\bf Abnormal init}
%     & Success $\uparrow$ \\
%     & Reward  $\uparrow$ \\
%     & Steps $\downarrow$ \\
% \midrule
% \multirow{3}{*}{\bf Abnormal final}
%     & Success $\uparrow$ \\
%     & Reward  $\uparrow$ \\
%     & Steps $\downarrow$ \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table*}




















\begin{table*}[t]
\caption{\small{Comparisons of the proposed method and baselines on different testing subsets. Each experiment is performed 5 times with different random seeds, average results are reported.}}
\vspace{-10pt}
\label{tbl:baselines_generalization}
\begin{center}
\small
\setlength{\tabcolsep}{3pt}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
& \multicolumn{3}{c}{\bf Normal } &  \multicolumn{3}{c}{\bf Less subgoals } & \multicolumn{3}{c}{\bf More subgoals } \\
\midrule
& Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ \\
\midrule
OG-1 MLP  & 25.840  & 3.673 & 85.463	& 64.000  & 1.280 & 52.576	& 7.400 &  6.052 & 97.662  \\
OG-N MLP  & 27.040 & 4.214 & 87.355 &	70.400 & 1.408 & 50.924	& 6.000 & 6.484 & 98.638	 \\
OG-1 LSTM  & 38.760 & 5.586 & 76.471	& 63.600 & 1.272 & 45.718	& 21.500 & 9.998 & 91.689	 \\
\midrule
OG LM  (scratch) & 	60.560 & 6.523 & 66.815	& 95.600 & 1.916 & 21.414	& 30.800 & 11.488 & 91.493	 \\
\midrule
% OGM LM  (scratch) & 69.200 & 7.092 & 60.000	& 94.000 & 1.880 & 19.050	& 28.500 & 12.400 & 91.140	 \\
% \midrule
OG LM (ft) & 62.720 & 6.447 & 60.406	& 93.600 & 1.872 & 19.356	& 43.000 & 11.632 & 82.290		\\
\midrule
OGM LM  (scratch) & 69.200 & 7.092 & 60.000	& 94.000 & 1.880 & 19.050	& 28.500 & 12.400 & 91.140	 \\
\midrule
OGM LM (ft) & 76.160 & 7.164 & 51.572	& 98.200 & 1.964 & 14.512	& 48.500 & 12.514 & 80.873  \\
\midrule
% OGM LM (ft) & 71.520 & 7.003 & 55.895	& 95.800 & 1.916 & 17.968	& 52.300 & 12.822 & 79.233	 \\
% \midrule
&  \multicolumn{3}{c}{\bf Zero-shot } & \multicolumn{3}{c}{\bf Abnormal } & \multicolumn{3}{c}{\bf Zero-shot + Abnormal } \\
\midrule
& Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ \\
\midrule
OG-1 MLP  &  7.600  &  1.772 & 96.562    & 32.400  & 4.032 & 78.432	& 4.600 &   1.084 & 97.782 \\
OG-N MLP  & 7.200 & 2.712 & 96.668 &	31.000 & 3.464 & 85.950	& 4.800 & 2.588 & 97.210 \\
OG-1 LSTM  & 0.000 & 0.112 & 100.000	& 20.000 & 3.232 & 90.416	& 0.400  & 0.184 & 99.802 \\
\midrule
OG LM  (scratch) & 0.200 & 0.100 & 99.982	& 62.800 & 5.284 & 68.440	& 2.200 & 0.320 & 98.882	\\
\midrule
% OGM LM  (scratch) &  2.000 & 0.220 & 99.320	& 69.000 & 5.560 & 60.680	& 4.000 & 0.520 & 97.780 \\
% \midrule
OG LM (ft) & 23.800 & 3.108 & 86.158	& 63.800 & 5.256 & 62.780	& 26.200 & 3.248 & 84.234	\\
\midrule
OGM LM  (scratch) &  2.000 & 0.220 & 99.320	& 69.000 & 5.560 & 60.680	& 4.000 & 0.520 & 97.780 \\
\midrule
OGM LM (ft) & 21.800 & 3.152 & 87.620	& 79.200 & 5.840 & 50.566	& 27.000 & 3.324 & 84.380  \\
\midrule
% OGM LM (ft) & 29.200 & 3.780 & 83.772	 & 69.200 & 5.548 & 57.184	 & 29.800 & 3.720 & 83.758 \\
% \bottomrule
\end{tabular}
}
\end{center}
\end{table*}










==> table/result1.tex <==

\begin{table*}[t]
\caption{\small{does LM pretraining help?}}
\vspace{-5pt}
\label{tbl:result1}
\begin{center}
\small
\setlength{\tabcolsep}{3pt}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
& \multicolumn{3}{c}{\bf Normal } &  \multicolumn{3}{c}{\bf Less subgoals } & \multicolumn{3}{c}{\bf More subgoals } \\
\midrule
& Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ \\
\midrule
OG-1 LSTM  & 38.760 & 5.586 & 76.471	& 63.600 & 1.272 & 45.718	& 21.500 & 9.998 & 91.689	 \\
\midrule
OGM LM  (scratch) & 69.200 & 7.092 & 60.000	& 94.000 & 1.880 & 19.050	& 28.500 & 12.400 & 91.140	 \\
\midrule
OGM LM (ft) & 76.160 & 7.164 & 51.572	& 98.200 & 1.964 & 14.512	& 48.500 & 12.514 & 80.873  \\
\midrule
&  \multicolumn{3}{c}{\bf Zero-shot } & \multicolumn{3}{c}{\bf Abnormal } & \multicolumn{3}{c}{\bf Zero-shot + Abnormal } \\
\midrule
& Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ \\
\midrule
OG-1 LSTM  & 0.000 & 0.112 & 100.000	& 20.000 & 3.232 & 90.416	& 0.400  & 0.184 & 99.802 \\
\midrule
OGM LM  (scratch) &  2.000 & 0.220 & 99.320	& 69.000 & 5.560 & 60.680	& 4.000 & 0.520 & 97.780 \\
\midrule
OGM LM (ft) & 21.800 & 3.152 & 87.620	& 79.200 & 5.840 & 50.566	& 27.000 & 3.324 & 84.380  \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}














==> table/result2.tex <==

\begin{table*}[t]
\caption{\small{in what part of the model is pretraining most important?}}
\vspace{-5pt}
\label{tbl:ablation}
\begin{center}
\small
\setlength{\tabcolsep}{3pt}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
& \multicolumn{3}{c}{\bf Normal } &  \multicolumn{3}{c}{\bf Less subgoals } & \multicolumn{3}{c}{\bf More subgoals } \\
\midrule
& Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ \\
\midrule
OGM LM (ft) & 76.160 & 7.164 & 51.572	& 98.200 & 1.964 & 14.512	& 48.500 & 12.514 & 80.873  \\
\midrule
OGM LM (ft) - OLF & 62.000 & 5.652 & 59.784	& 80.000 & 1.600 & 30.460	& 46.000 & 10.470 & 83.190		 \\
\midrule
OGM LM (ft) - GLF & 67.600 & 6.460 & 58.982	& 79.000 & 1.580 & 32.500	& 45.000 & 11.610 & 85.570	 \\
\midrule
OGM LM (ft) - MLF &  61.800 & 5.592 & 61.196	& 76.000 & 1.520 & 36.480	& 40.500 & 10.140 & 86.525	 \\
\midrule
&  \multicolumn{3}{c}{\bf Zero-shot } & \multicolumn{3}{c}{\bf Abnormal } & \multicolumn{3}{c}{\bf Zero-shot + Abnormal } \\
\midrule
& Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ \\
\midrule
OGM LM (ft) & 21.800 & 3.152 & 87.620	& 79.200 & 5.840 & 50.566	& 27.000 & 3.324 & 84.380  \\
\midrule
OGM LM (ft) - OLF & 19.000 & 2.860 & 89.470	& 72.000 & 5.580 & 50.140		 & 27.000 & 3.240 & 85.180 \\
\midrule
OGM LM (ft) - GLF & 84.000 & 6.100 & 54.920	& 84.000 & 5.980 & 48.170	& 66.000 & 5.260 & 66.250 \\
\midrule
OGM LM (ft) - MLF & 36.000 & 4.380 & 79.340	& 82.000 & 6.000 & 47.230	& 67.000 & 5.640 & 63.930 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}

















==> table/result3.tex <==

\begin{table*}[t]
\caption{\small{do language-based encodings actually matter?}}
\vspace{-5pt}
\label{tbl:result3}
\begin{center}
\small
\setlength{\tabcolsep}{3pt}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
& \multicolumn{3}{c}{\bf Normal } &  \multicolumn{3}{c}{\bf Less subgoals } & \multicolumn{3}{c}{\bf More subgoals } \\
\midrule
& Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ \\
\midrule
OGM LM (ft) & 76.160 & 7.164 & 51.572	& 98.200 & 1.964 & 14.512	& 48.500 & 12.514 & 80.873  \\
\midrule
OGM LM (ft) (random) & 78.960 & 6.978 & 49.824	& 94.200 & 1.884 & 18.480	& 51.500 & 12.446 & 82.337	 \\
\midrule
&  \multicolumn{3}{c}{\bf Zero-shot } & \multicolumn{3}{c}{\bf Abnormal } & \multicolumn{3}{c}{\bf Zero-shot + Abnormal } \\
\midrule
& Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ & Success $\uparrow$ & Reward $\uparrow$ & Steps $\downarrow$ \\
\midrule
OGM LM (ft) & 21.800 & 3.152 & 87.620	& 79.200 & 5.840 & 50.566	& 27.000 & 3.324 & 84.380  \\
\midrule
OGM LM (ft) (random) & 22.600 & 2.500 & 87.444	& 88.400 & 6.164 & 42.782	& 33.600 & 3.248 & 81.446 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}
















==> table/tasks.tex <==


\begin{table*}
\caption{\small{}}
\label{tbl:ablations}
\begin{center}
\small
\setlength{\tabcolsep}{3pt}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|cccc|cccc}
\toprule
& \multicolumn{4}{c|}{\bf Single Agent} & \multicolumn{4}{c}{\bf Multi-agent} \\
\midrule
Task names & Set Table & Put Groceries & Set Meal & Wash Dishes & Set table & Put groceries & Set meal & Wash dishes  \\
\midrule
\# Subgoals & $3\sim8$  & $3\sim8$  & $3\sim8$  & $3\sim8$  & $3\sim8$  & $3\sim8$  & $3\sim8$  & $3\sim8$  \\
\# Trajectories & \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


set table:

Put Groceries:
put object into fridge

wash dishes:
dishwasher

read book:
bring some object into a coffeetable, find the book and set next to object


unseen task category:
set meal:
put food on table




Tasks:
what tasks we have now
what tasks are good for multi-agents



Generalization:

unseen task category: set meal
unseen task combinations: seen categories, the combination are different (2 plates, 2 forks) (1 plate, 1 fork)

combined tasks (setup table + read book)
unseen task number: subgoals 2-6, testing > 6


unseen object positions
unseen object category
less objects
more objects

unseen actions


Nature and abnormal for human:
object distribution is abnormal
tasks are abnormal


initial belief of agent


can I open several xserver on visiongpus.
